WISE: A Framework for Gigapixel Whole-Slide-Image Lossless Compression

Whole-Slide Images (WSIs) have revolutionized medical analysis by presenting high-resolution images of the whole tissue slide. Despite avoiding the physical storage of the slides, WSIs require considerable data volume, which makes the storage and maintenance of WSI records costly and unsustainable. To this end, this work presents the first investigation of lossless compression of WSI images. Interestingly, we find that most existing compression methods fail to compress the WSI images effectively. Furthermore, our analysis reveals that the failure of existing compressors is mainly due to information irregularity in WSI images. To resolve this issue, we developed a simple yet effective lossless compressor called WISE, specifically designed for WSI images. WISE employs a hierarchical encoding strategy to extract effective bits, reducing the entropy of the image and then adopting a dictionary-based method to handle the irregular frequency patterns. Through extensive experiments, we show that WISE can effectively compress the gigapixel WSI images to 36 times on average and up to 136 times.

==> sec/2_Motivation.tex <==
\section{Motivation}
\label{sec:motivation}
%Current compression method fail on WSI images, even though there's quite a need to compressed and store them. 
%Since C16 and C17's images contains a huge amount of black area, we extract the information area in C16 and C17 to conduct this motivation experiment. The compression ratio is calculated using the following formula:

% \begin{equation}
% \text { compression ratio }=\frac{\text { size of uncompressed data }}{\text { size of compressed data }}
% \end{equation}

\begin{table}[t]
  \caption{Compression ratio on 256x256 WSI patches on TCGA, C16, and C17.}
  \label{tab:comp_motiv}
  \centering
  \begin{tabular}{|l|l|ccc|}
    \hline
    \multicolumn{5}{|c|}{\textbf{Traditional Compressor}} \\
    \hline
     & & \textbf{TCGA} & \textbf{C16} & \textbf{C17} \\
    \hline
    Dictionary-based & Gzip & 1.04 & 1.02 & 1.09\\
    Integer-based & Simple8b & 1.04 & 1.02 & 1.09\\
    Image-based & PNG & 1.04 & 1.02 & 1.09\\
    Entropy-based & Huffman & 1.14 & 1.09 & 1.19\\
    %FSE & & & \\
    \hline
    \multicolumn{5}{|c|}{\textbf{NN-based Compressor}} \\
    \hline
    % PAC & 1.01 & 1.02 & 1.09\\
    Byte-stream-based & NNCP & 2.29 & 1.32 & 2.09\\
    % \hline
    % \multicolumn{4}{|c|}{\textbf{NN-based Image Compressor}} \\
    % \hline
    Image-based & ArIB-BPS & 1.64 & 1.61 & 1.61\\
    \hline
    %\multicolumn{5}{|c|}{\textbf{NN-based Byte-Stream Compressor}}\\
     \multicolumn{2}{|c|}{\textbf{\ours}}  & 1.64 & 1.61 & 1.61\\
    \hline
  \end{tabular}
\end{table}

Essentially, the success of many compression methods relies on identifying the locality properties within adjacent pixels or the pixel value distributions.
Nevertheless, WSI images may demonstrate a different locality pattern from normal images such that existing compression methods fail to achieve satisfactory performance.
% Most compression methods are based on adjacent pixel correlations or pixel value distributions. However, directly applying these compression method on WSI pixels would not yield satisfied compression performance. 


\begin{figure}[t]
  \centering
\includegraphics[width=0.45\textwidth,angle=0]{figures/motivation.pdf}
  \caption{WSI image's pixel intensity variation is quite different from normal image. It has a large portion of high-frequency features thus affecting the performance of entropy-based compressors.}
\label{fig:freq_analysis}
\end{figure}

To begin with our analysis, we start by conducting an empirical study on the data \yq{WHAT concrete data?}. The results are given in Table~\ref{tab:comp_motiv}. Specifically, we consider $6$ prevalent compression methods, including traditional compressors like Huffman~\citep{huffman1952method}, FSE~\yq{CITE}, pfor~\yq{??}, PAC~\yq{??}, PNG~\citep{png}, and LZMA~\yq{??}, as well as neural network based compressors like NNCP~\yq{CITE} and ArIB-BPS~\yq{CITE}.
%
% We conduct an empirical study on the data provided in Fig.~\ref{fig:freq_analysis} to illustrate this problem. In Tab.~\ref{tab:empirical} we employ six different compression algorithms: Huffman, FSE, pfor, PAC, PNG, and LZMA. 
%
The compression ratio values reflect the effectiveness of each algorithm in reducing WSI image size, where higher values generically indicate better compression performance for the given data. 
%
\yq{TODO: Table 1 and 2 seem not aligned}
We can see that PNG achieves the highest compression ratio for normal images but has barely no compression ratio on WSI images. On the contrary, dictionary-based method lzma yeilds relatively high compresstion ratio on WSI images. We concluded that this is because dictionary-based method can directly capture \hl{WSI's high-frequency feature patterns, which is hard to predict through entropy coding and predictive coding but can be directly extract from historical experience.} However, a near 2x compression ratio remains sufficient for WSI slides, which often reach sizes of several gigabytes. Therefore, dictionary-based methods still offer significant potential for optimization.

To better understand the failure reasons of the existing compression methods. We further analyze the characteristics of the WSI images. As the identification of locality properties has been shown to be quite sensitive to the frequency patterns in the input data~\citep{rhee2022lc}, we focus on analyzing the frequency characteristics of the WSI images.
% The reason for WSI's bad compression ratio is its distinct feature characteristics, which we defined as \textit{information irregularity}. WSI's information irregularity displays at two aspects: irregular high-frequency features and irregular local extremes. 
%
As illustrated in Fig.~\ref{fig:freq_analysis}, compared with normal images, WSI images demonstrate unique properties in the frequency domain, which we term as \textit{information irregularity}.
Specifically, the frequency information in the WSI images consists of a large part of the high-frequency features, as well as more local extremes. The \textit{high volatility} of the WSI data poses a significant challenge to effectively capturing the locality for compression, especially for prediction-based compressors~\yq{CITE}.
% This trait poses a challenge for compression tasks, leading to failures in all prediction-based compressors which is originally designed for normal images. High frequency features is recognized as very difficult to compress, as shown in recent papers~\cite{rhee2022lc}. 

Table~\ref{tab:empirical} presents the direct head-to-head comparison of performances of existing compressors on both normal image data and the WSI image data.
Specifically, the best compressor for normal image data, PNG, can only achieve little-to-no compression ratio on WSI images. On the contrary, the dictionary-based method lzma yields a relatively high compression ratio on WSI images. 
The same phenomenon happens to the other compressors such as Huffman, Pfor, and PAC.
%
Nevertheless, the simple dictionary-based compression method LZMA can achieve relatively high compression ratios on both normal and WSI images. \hl{The reason is that constructing a dictionary instead of predicting the sequential patterns is more robust to the high volatility of the WSI data. } 
% We concluded that this is because the dictionary-based method can directly capture \hl{WSI's high-frequency feature patterns, which is hard to predict through entropy coding and predictive coding but can be directly extract from historical experience.} 
However, a near 2x compression ratio remains sufficient for WSI slides, which often reach sizes of several gigabytes. 
% Therefore, dictionary-based methods still offer significant potential for optimization.


%for which is hard to capture through entropy coding and predictive coding. 

%For Normal Images, PNG achieves the highest compression ratio at 2.06, followed by PAC at 1.98 and LZMA at 1.43.
%For WSI Images, LZMA provides the highest compression ratio of 1.93, while PAC achieves the lowest at 0.87.
%Interestingly, Huffman and FSE show identical compression ratios for WSI Images (1.23), indicating similar performance in this data type.
\begin{table}[t]
\centering
\caption{Empirical Study for Normal and WSI Images. \yq{TODO: aligning to Table 1; check whether it's needed to include \ours; details of the data}}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
 & \textbf{Huffman}  & \textbf{Pfor} & \textbf{PAC} & \textbf{PNG} & \textbf{LZMA} \\
\hline
\textbf{Normal} & 1.19  & 1.42 & 1.98 & 2.06 & 1.43 \\
\textbf{WSI} & 1.23  & 0.99 & 0.87 & 1.01 & 1.93 \\
\hline
\end{tabular}
\label{tab:empirical}
\end{table}



%Tab.~\ref{tab:comp_motiv} demonstrates that nearly all compressors struggle to effectively compress WSI images. While Huffman coding, FSE, and ArIB-BPS achieve minimal compression, PAC and NNCP fail to capture the underlying data distribution entirely. Notably, ArIB-BPS can achieve a compression ratio of 1.5x. However, the NN-based image compressor is relatively expensive, requiring \hl{xx} seconds to compress a single image, rendering it impractical for real-world applications. Moreover, this compression ratio is insufficient for long-term storage needs.



% Entropy-based method's failure is due to the unique pixel distribution characteristics of WSI images. The WSI image's pixel distribution has two main characteristics: 1. The pixel value is approximately uniform distributed in feature space. 2. WSI is full of high frequency features across the image. High frequency features is recognized as very difficult to compress, as shown in recent papers~\cite{rhee2022lc}. 

% MOVE TO NEXT SECTION
% In this paper we propose a dictionary-based compression method to conquer this issue. We first split the empty and non-empty area of WSI images, and compress them separately. For non-empty area of WSI images, a delta method is introduced to enhance the compression ratio. Additionally, a bitmap split algorithm is designed to compress each bit position in WSI images separately. 






==> tables/compression_full.tex <==
\begin{table*}[t]
	\centering
\caption{Compression results on entire gigabytes whole-slide images.}
\label{tab:compression_results_full}
% \resizebox{\textwidth}{!}{
	% \small
	\begin{tabular}{l*{6}{p{1.8cm}}}
		\toprule
							         & {\small  C16 ($\uparrow$)} & {\small C17($\uparrow$)} & {\small TCGA($\uparrow$)} & {\small BNCB($\uparrow$)}& {\small DigestPath($\uparrow$)}& {\small IHC4BC($\uparrow$)} \\\midrule
		Huffman                 & $3.10$                     & $4.41$                    & $1.88$                     & $1.12$                    & $1.07$                    & $1.45$                     \\\hdashline[0.5pt/1pt]
		%FSE                 &               & $00.00$                     & $00.00$                    & $3.16$                     & $1.46$                    & $00.00$                    & $00.00$                     \\\hdashline[0.5pt/1pt]
		\rule{0pt}{10pt}PNG                  & $5.15$                     & $9.14$                    & $3.16$                     & $1.46$                    & $7.32$                    & $2.75$                     \\
		TIFF                  & $8.00$                     & $14.23$                    & $4.35$                     & $1.16$                    & $1.18$                    & $2.32$                     \\\hdashline[0.5pt/1pt]
		\rule{0pt}{10pt}Gzip             & $9.47$                     & $18.34$                    & $4.72$                     & $1.15$                    & $1.17$                    & $2.00$                     \\
	%	Gzip             & $\checkmark$ & $00.00$                     & $00.00$                    & $00.00$                     & $00.00$                    & $00.00$                    & $00.00$                     \\
		%7z              &              & $00.00$                     & $00.00$                    & $00.00$                     & $00.00$                    & $00.00$                    & $00.00$                     \\
		  %7z              & $\checkmark$ & $00.00$                     & $00.00$                    & $00.00$                     & $00.00$                    & $00.00$                    & $00.00$                     \\
            Lzma & $14.60$                     & $26.09$                    & $6.60$                     & $1.29$                    & $1.56$                    & $2.60$                     \\
            Zstd & $14.60$                     & $23.28$                    & $6.60$                     & $1.29$                    & $1.56$                    & $2.60$                     \\
		  \ours                 & $00.00$                     & $36.11$                    & $00.00$                     & $1.63$                    & $2.50$                    & $3.85$                     \\
		% ArIB-BPS             &              & $00.00$                     & $00.00$                    & $00.00$                     & $00.00$                    & $00.00$                    & $00.00$                     \\
		% ArIB-BPS             & $\checkmark$ & $00.00$                     & $00.00$                    & $00.00$                     & $00.00$                    & $00.00$                    & $00.00$                     \\
            \bottomrule
		\multicolumn{5}{l}{$^\uparrow$The higher number indicates better compression performance.}                                                                                                                                                                                                                                                                                                                                                                                                                             \\                                                                                                                                                                                                                                                                                                                                           \\
	\end{tabular}%}
\end{table*}
